On Verifying Resource Contracts using Code Contracts

In this paper we present an approach to check resource consumption contracts using an off-the-shelf static analyzer. We propose a set of annotations to support resource usage specifications, in particular, dynamic memory consumption constraints. Since dynamic memory may be recycled by a memory manager, the consumption of this resource is not monotone. The specification language can express both memory consumption and lifetime properties in a modular fashion. We develop a proof-of-concept implementation by extending Code Contracts' specification language. To verify the correctness of these annotations we rely on the Code Contracts static verifier and a points-to analysis. We also briefly discuss possible extensions of our approach to deal with non-linear expressions.

==> eptcsdata.tex <==
\providecommand{\firstpage}{1}
\providecommand{\publicationstatus}{Nazareno Aguirre, Leila Ribeiro (Eds.):\\
First Latin American Workshop on Formal Methods (LAFM 2013)\\
EPTCS 139, 2014, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.139.1}{10.4204/EPTCS.139.1}}
\pdfoutput=1

